Making Convolutional Networks Shift-Invariant Again

Modern convolutional networks are not shift-invariant, as small input shifts or translations can cause drastic changes in the output. Commonly used downsampling methods, such as max-pooling, strided-convolution, and average-pooling, ignore the sampling theorem. The well-known signal processing fix is anti-aliasing by low-pass filtering before downsampling. However, simply inserting this module into deep networks degrades performance; as a result, it is seldomly used today. We show that when integrated correctly, it is compatible with existing architectural components, such as max-pooling and strided-convolution. We observe \textit{increased accuracy} in ImageNet classification, across several commonly-used architectures, such as ResNet, DenseNet, and MobileNet, indicating effective regularization. Furthermore, we observe \textit{better generalization}, in terms of stability and robustness to input corruptions. Our results demonstrate that this classical signal processing technique has been undeservingly overlooked in modern deep networks. Code and anti-aliased versions of popular networks are available at https://richzhang.github.io/antialiased-cnns/ .

==> tables/results_cifar.tex <==
%\begin{table}[t]
%\scalebox{.85} {
% \begin{tabular}{c c c c c c c}
% \toprule
%
%& \multicolumn{6}{c}{{\bf VGG13-bn} \cite{simonyan2014very}} \\ \cmidrule(lr){2-7}
% \multirow{4}{*}{\bf Filter} & \multicolumn{3}{c}{\bf Train w/o augmentation} & \multicolumn{3}{c}{\bf Train w/ augmentation} \\ \cmidrule(lr){2-4} \cmidrule(lr){5-7}
% & \multicolumn{2}{c}{\bf Accuracy} & \multirow{2}{*}{\bf \shortstack[c]{Consist-\\ency}} & \multicolumn{2}{c}{\bf Accuracy} & \multirow{2}{*}{\bf \shortstack[c]{Consist-\\ency}} \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6}
% & {\bf None} & {\bf Rand} & & {\bf None} & {\bf Rand} & \\ \midrule
%{\bf Delta-1} & \worst{91.6} & \worst{87.4} & \worst{88.1} & 93.4 & \textbf{93.8} & \worst{96.6} \\   \cdashline{1-7}
%{\bf Rect-2} & 92.8 & \worst{89.3} & \worst{90.5} & \textbf{93.9} & 93.7 & \worst{97.6} \\
%{\bf Tri-3} & 93.1 & 91.4 & 93.9 & 93.6 & \best{93.6} & 98.0 \\
%{\bf Bin-4} & 93.0 & 91.1 & 93.2 & 93.4 & 93.2 & 98.1 \\
%{\bf Bin-5} & \textbf{93.2} & 92.6 & 96.3 & 93.1 & 93.2 & 98.4 \\
%{\bf Bin-6} & 93.0 & 92.4 & 96.9 & 93.4 & 93.4 & 98.6 \\
%{\bf Bin-7} & 93.0 & \textbf{93.0} & \textbf{98.1} & 93.2 & 93.2 & \textbf{98.8} \\   
%\bottomrule
%
%\vspace{-5mm}
%\end{tabular}
%}
%\vspace{-5mm}
%\caption{{\bf CIFAR Classification.} Results across blurring filters and training scenarios, without and with data augmentation. We evaluate classification accuracy without shifts ({\bf accuracy -- None}) and on random shifts ({\bf Accuracy -- Random}), as well as classification {\bf consistency}. Results are plotted in Fig.~\ref{fig:consist_vs_acc_cifar}.
%\vspace{-6mm}
%\label{tab:results-cifar}
%}
%\end{table}

\begin{table}[t]
\scalebox{1.} {
 \begin{tabular}{c c c c c c}
 \toprule

& & \multicolumn{4}{c}{\bf VGG13-bn} \\ \cmidrule(lr){3-6}
\multirow{2}{*}{\bf Method} & \multirow{2}{*}{\bf Filter} & \multicolumn{2}{c}{\bf Train w/o aug} & \multicolumn{2}{c}{\bf Train w/ aug} \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6}
& & \bf Acc & \bf Con & \bf Acc & \bf Con \\ \midrule
% & {\bf None} & {\bf Rand} & & {\bf None} & {\bf Rand} & \\ \midrule
{\bf Baseline} & {\bf Delta-1} & \worst{91.6} & \worst{88.1} & \textbf{93.8} & \worst{96.6} \\   \cdashline{1-6}
\multirow{6}{*}{\bf \shortstack[c]{Anti-\\Aliased}} & {\bf Rect-2} & 92.8 & \worst{90.5} & 93.7 & \worst{97.6} \\
& {\bf Tri-3} & 93.1 & 93.9 & \best{93.6} & 98.0 \\
& {\bf Bin-4} & 93.0 & 93.2 & 93.2 & 98.1 \\
& {\bf Bin-5} & \textbf{93.2} & 96.3 & 93.2 & 98.4 \\
& {\bf Bin-6} & 93.0 & 96.9 & 93.4 & 98.6 \\
& {\bf Bin-7} & 93.0 & \textbf{98.1} & 93.2 & \textbf{98.8} \\   
\bottomrule
\vspace{-5mm}
\end{tabular}
}
\vspace{-4mm}
\caption{{\bf CIFAR Classification.} We evaluate accuracy ({Acc}) and consistency ({Con}), using progressively larger anti-aliasing filters. We evaluate the network, training both without and with shift-based data augmentation. Results are plotted in Fig.~\ref{fig:consist_vs_acc_cifar}.
\vspace{-6mm}
\label{tab:results-cifar}
}
\end{table}


==> tables/results_imagenet.tex <==

\begin{table}[t]
\scalebox{.8} {
 \begin{tabular}{c c c c c c c c c}
 \toprule
& \multicolumn{8}{c}{\bf ImageNet Classification} \\ \cmidrule(lr){2-9}
\multirow{2}{*}{\bf Filter} & \multicolumn{2}{c}{\bf AlexNet} & \multicolumn{2}{c}{\bf VGG16} & \multicolumn{2}{c}{\bf ResNet50} & \multicolumn{2}{c}{\bf DenseNet121} \\
% & & & \multicolumn{2}{c}{\bf 50} & \multicolumn{2}{c}{\bf Net121} \\
%%& \multicolumn{4}{c}{\cite{krizhevsky2012imagenet}} & \multicolumn{4}{c}{\cite{simonyan2014very}} & \multicolumn{4}{c}{\cite{He_2016_CVPR}} & \multicolumn{4}{c}{\cite{huang2017densely}}
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
%
 & {\bf Acc} & {\bf Con} & {\bf Acc} & {\bf Con} & {\bf Acc} & {\bf Con} & {\bf Acc} & {\bf Con} \\ \midrule

{\bf Baseline}
& 56.5& 78.2
& 71.6& 88.5
& 76.2& 89.2
& 74.4& 88.8
\\
\cdashline{1-9}
{\bf Rect-2}
& {\bf 57.2}& 81.3
& 72.2& 89.2
& 76.8& 90.0
& 75.0& 89.5
\\
{\bf Tri-3}
& 56.9& 82.2
& 72.2& 89.6
& 76.8& 90.9
& {\bf 75.1}& 89.8
\\
{\bf Bin-5}
& 56.6& {\bf 82.5}
& {\bf 72.3}& {\bf 90.2}
& {\bf 77.0}& {\bf 91.3}
& 75.0& {\bf 90.4}
\\



\bottomrule

\vspace{-5mm}
\end{tabular}
}
\vspace{-5mm}
\caption{{\bf Imagenet Classification.} We show 1000-way classification accuracy and consistency (higher is better), across 4 architectures, with our anti-aliasing filtering added. We test 3 filters, in addition to the off-the-shelf models. As designed, classification consistency is improved across all methods.  Interestingly, accuracy is \textit{also improved}. We recommend \textit{Tri-3} or \textit{Bin-5} for general use.
\vspace{-4mm}
\label{tab:results-imagenet}
}
\end{table}


==> tables/results_submission.tex <==
\begin{table}
\scalebox{.6} {
 \begin{tabular}[t]{c c c c c c c c c c c c}
 \toprule
\multirow{3}{*}{\bf Filter shape} & \multirow{3}{*}{\bf \# Taps} & \multirow{3}{*}{\bf Weights} & \multicolumn{4}{c}{\bf Train with no augmentation} & \multicolumn{4}{c}{\bf Train with Augmentation} \\ \cmidrule(lr){4-7} \cmidrule(lr){8-11}

 &  &  & \multicolumn{2}{c}{\bf Test accuracy} & {\bf Classification} & \multirow{ 2}{*}{\bf Average} \hspace{2mm} & \hspace{2mm} \multicolumn{2}{c}{\bf Test accuracy} & {\bf Classification} & \multirow{2}{*}{\bf Average} \\ \cmidrule(lr){4-5} \cmidrule(lr){8-9}

 &  &  & {\bf None} & {\bf Random} & {\bf Consistency} & & {\bf None} & {\bf Rand} & {\bf Consistency} & \\ \midrule

{\bf Delta (baseline)} & 1 & [1] & 91.6\% & 87.5\% & 88.1\% & \colorbox{pink}{89.9\%} & 93.4\% & 93.8\% &  96.6\% & \colorbox{pink}{95.0\%} \\  \midrule

{\bf Rectangle} & 2 & [1, 1] & 92.8\% & 89.2\% & 90.5\% & \colorbox{pink}{91.6\%} & 93.9\% & 93.7\% & 97.6\% & 95.8\% \\


{\bf Rectangle} & 3 & [1, 1, 1] & 93.4\% & 91.9\% & 94.5\% & 93.9\% & 93.6\% & 93.7\% & 97.9\%& 95.7\% \\


{\bf Rectangle} & 4 & [1, 1, 1, 1] & 93.2\% & 92.8\% & 97.7\% & 95.4\% & 93.4\% & 93.4\% & 98.5\% & 95.9\% \\


{\bf Rectangle} & 5 & [1, 1, 1, 1, 1] & 92.2\% & 92.0\% & 98.3\% & 95.2\% & 92.4\% & 92.6\% & 98.7\% & 95.6\% \\


{\bf Rectangle} & 6 & [1, 1, 1, 1, 1, 1] & 91.4\% & 91.3\% & 97.3\% & 94.4\% & 91.4\% & 91.4\% & 98.9\%& \colorbox{pink}{95.2\%} \\


{\bf Rectangle} & 7 & [1, 1, 1, 1, 1, 1, 1] & 90.8\% & 90.7\% & 98.8\% & 94.8\% & 90.5\% & 90.6\% & 99.0\% & \colorbox{pink}{94.8\%} \\  \midrule


{\bf Triangle} & 3 & [1, 2, 1] & 93.1\% & 91.7\% & 93.9\% & 93.5\% & 93.6\% & 93.6\% & 98.0\% & 95.8\% \\


\cellcolor{lightyellow}{\bf Triangle} & \cellcolor{lightyellow}{5} & \cellcolor{lightyellow}{[1, 2, 3, 2, 1]} & 93.3\% & 93.3\% & 98.2\% & \colorbox{lightgreen}{95.7\%} & 93.3\% & 93.3\% & 98.6\% & \colorbox{lightgreen}{96.0\%} \\


{\bf Triangle} & 7 & [1, 2, 3, 4, 3, 2, 1] & 92.3\% & 92.3\% & 98.8\% & \colorbox{lightgreen}{95.5\%} & 92.4\% & 92.3\% & 99.0\% & 95.7\% \\   \midrule


{\bf Pascal} & 4 & [1, 3, 3, 1] & 93.0\% & 91.5\% & 93.2\% & 93.1\% & 93.4\% & 93.2\% & 98.1\% & 95.7\% \\


{\bf Pascal} & 5 & [1, 4, 6, 4, 1] & 93.2\% & 92.2\% & 96.3\% & 94.8\% & 93.1\% & 93.2\% & 98.4\% & 95.8\% \\


{\bf Pascal} & 6 & [1, 5, 10, 10, 5, 1] & 93.0\% & 92.3\% & 96.9\% & 94.9\% & 93.4\% & 93.4\% & 98.6\% & \colorbox{lightgreen}{96.0\%} \\


\cellcolor{lightyellow}{\bf Pascal} & \cellcolor{lightyellow}{7} & \cellcolor{lightyellow}{[1, 6, 15, 20, 15, 6, 1]} & 93.0\% & 93.0\% & 98.1\% & \colorbox{lightgreen}{95.5\%} & 93.2\% & 93.2\% & 98.8\% & \colorbox{lightgreen}{96.0\%} \\   \midrule


{\bf Window} & 3 & [1, 1.57, 1] & 93.3\% & 91.5\% & 94.2\% & 93.8\% & 93.5\% & 93.6\% & 98.0\% & 95.7\% \\


{\bf Window} & 6 & [-1, 1.67, 5, 5, 1.67, -1] & 92.9\% & 90.2\% & 91.4\% & \colorbox{pink}{92.1\%} & 93.4\% & 93.5\% & 98.1\% & 95.7\% \\


{\bf Window} & 7 & [-1, 0, 3, 4.71, 3, 0, -1] & 92.4\% & 91.5\% & 94.0\% & 93.2\% & 93.4\% & 93.5\% & 97.8\% & 95.6\% \\   \midrule


{\bf Least Squares} & 3 & [1, 1,63, 1] & 93.1\% & 91.5\% & 93.8\% & 93.4\% & 93.7\% & 93.8\% & 98.0\% & 95.9\% \\



{\bf Least Squares} & 7 & [-1, 0, 3.80, 6.13, 3.80, 0, -1] & 92.7\% & 91.2\% & 93.9\% & 93.3\% & 93.4\% & 93.6\% & 97.9\% & 95.6\% \\

\bottomrule

\vspace{-7mm}
\end{tabular}
}
\caption{{\bf Results} We show results across blurring filters and training scenarios (without and with data augmentation). We evaluate on classification accuracy without shifts ({\bf Test accuracy -- none}) and on random shifts ({\bf Test accuracy -- Random}), as well as {\bf classification consistency}. We also compute an {\bf average} of test accuracy (without shifting) and classification consistency and highlight \colorbox{lightgreen}{top} and\colorbox{pink}{bottom} 3 performers. We use standard low-pass filters (note that weights are normalized to sum to 1): {\bf Rectangle} -- a moving average over neighboring values, {\bf Triangle} linearly decreases weight of neighbor values, {\bf Pascal} -- [1, 1] filter convolved with itself repeatedly, {\bf Window} -- filter produced using the window method (\texttt{firwin}) and {\bf Least Squares} error minimization (\texttt{firls}), from Python \texttt{scipy.signal} toolbox. \colorbox{lightyellow}{Triangle-5} and \colorbox{lightyellow}{Pascal-7} perform well across metrics, as more clearly seen in Fig.~\ref{fig:consist_vs_acc}}.
\vspace{-6mm}
\label{tab:results}
}
\end{table}





==> tables/testbeds.tex <==
%\begin{table}[h]
%\scalebox{.75} {
% \begin{tabular}{c c c c}
% \toprule
%  \multirow{2}{*}{\bf Network} & \multicolumn{2}{c}{\bf CIFAR10 Class.} & {\bf Labels$\rightarrow$Facades} \\  \cmidrule(lr){2-3} \cmidrule(lr){4-4}
% & VGG & DenseNet & U-Net \\ \cmidrule(lr){1-1} \cmidrule(lr){2-4}
% {\bf Train/Test size} & \multicolumn{2}{c}{50k/10k} & 400/106 \\ 
% {\bf Input} & \multicolumn{2}{c}{32$\times$32 image} & 256$\times$256 labels \\
% {\bf Output} & \multicolumn{2}{c}{classification} & 256$\times$256 image \\ 
% {\bf Loss function} & \multicolumn{2}{c}{cross-entropy} & {L1+GAN} \\
%  \cdashline{1-1} \cdashline{2-4}
% {\bf Down layers} & 5 & 2 & 7 \\
%% layers & & & \\ 
% {\bf Baseline method} & \multirow{1}{*}{MaxPool} & \multirow{1}{*}{AvgPool} & \multirow{1}{*}{StridedConv} \\
% {\bf Our replacement} & MaxBlurDown & BlurDown & ConvBlurDown \\
%\bottomrule
%\vspace{-11mm}
%\end{tabular}
%}
%\caption{{\bf Testbeds.} We test across tasks and architectures. Each downsamples differently, in terms of method and number of downsampling layers. Our method is compatible with each variant.
%\vspace{-7mm}
%\label{tab:testbeds}
%}
%\end{table}

%\begin{table*}[h]
%\scalebox{.74} {
% \begin{tabular}{c c c c}
% \toprule
%\multirow{2}{*}{\bf Tasks} & {\bf ImageNet} & {\bf CIFAR10} & {\bf Labels} \\
% & {\bf Classification} & {\bf Classification} & {\bf $\rightarrow$Facades} \\ \cmidrule(lr){1-4}
% {\bf Train size} & 1.2M & 50k & 400 \\ 
%  {\bf Test size} & 50k & 10k & 106 \\ 
% {\bf Input} & 224$\times$224 img & 32$\times$32 img & 256$\times$256 labels \\
% {\bf Output} & 1000-way class & 10-way class & 256$\times$256 image \\ 
% {\bf Loss function} & cross-entropy & cross-entropy & L1+GAN \\
%
%\bottomrule
%\vspace{-11mm}
%\end{tabular}
%}
%\caption{{\bf Tasks.} To test the generality of our method, we test across tasks -- large-scale higher-resolution image classification, medium-scale low-resolution classification image, and small-scale conditional image generation.
%\label{tab:testbed-data}
%}
%\end{table}
%\quad

% ***** Only networks *****
%\begin{table*}[h]
%\scalebox{.9} {
% \begin{tabular}{c c c c c c c c}
% \toprule
%\multirow{4}{*}{\bf Architectures} & \multicolumn{4}{c}{\bf ImageNet} & \multicolumn{2}{c}{\bf CIFAR10} & {\bf L2F} \\
%%& & & \\
%\cmidrule(lr){2-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
%& {\bf Alex-} & {\bf VGG-} & {\bf Res-} & {\bf Dense-} & {\bf VGG-} & {\bf DenseNet} & {\bf U-} \\
%& {\bf Net} & {\bf 16} & {\bf Net50} & {\bf Net121} & {\bf 13bn} & {\bf 40-12} & {\bf Net} \\ \cmidrule(lr){1-8} % \cmidrule(lr){1-1} \cmidrule(lr){2-5} \cmidrule(lr){6-7} \cmidrule(lr){8-8}
%% layers & & & \\ 
%{\bf \# Downsamplings} & 4 & 5 & 5 & 5 & 5 & 2 & 7 \\ \cdashline{1-8}
%{\bf MaxPool} & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & -- & -- \\
%{\bf StridedConv} & $\checkmark$ & -- & $\checkmark$ & $\checkmark$ & -- & -- & $\checkmark$ \\
%{\bf AvgPool} & -- & -- & -- & $\checkmark$ & -- & $\checkmark$ & -- \\ % \cmidrule(lr){1-8}
%\bottomrule
%\vspace{-11mm}
%\end{tabular}
%}
%\caption{{\bf Testbeds (Tasks and Architectures).} To test the generality of our method, we test across tasks architectures. {\bf (Left)} We test different tasks -- ImageNet classification, CIFAR10 classification, and Labels$\rightarrow$Facades generation, which span different output types (images vs labels), resolutions (higher and lower-resolution), and dataset sizes. {\bf (Right)} We test across architectures. Each downsamples differently, in terms of number of downsampling layers (first row), and types of downsampling layers. Our method is compatible with each variant. As discussed in Section \ref{sec:our_method}, we make the following replacements: {\bf MaxPool$\rightarrow$MaxBlurPool}, {\bf StridedConv$\rightarrow$ConvBlurPool}, and {\bf AvgPool$\rightarrow$BlurPool}. 
%\label{tab:testbed}
%}
%\end{table*}


